A Survey of Multi-Tenant Deep Learning Inference on GPU

Deep Learning (DL) models have achieved superior performance. Meanwhile, computing hardware like NVIDIA GPUs also demonstrated strong computing scaling trends with 2x throughput and memory bandwidth for each generation. With such strong computing scaling of GPUs, multi-tenant deep learning inference by co-locating multiple DL models onto the same GPU becomes widely deployed to improve resource utilization, enhance serving throughput, reduce energy cost, etc. However, achieving efficient multi-tenant DL inference is challenging which requires thorough full-stack system optimization. This survey aims to summarize and categorize the emerging challenges and optimization opportunities for multi-tenant DL inference on GPU. By overviewing the entire optimization stack, summarizing the multi-tenant computing innovations, and elaborating the recent technological advances, we hope that this survey could shed light on new optimization perspectives and motivate novel works in future large-scale DL system optimization.

==> _txt/1_intro_bak.tex <==
\section{Introduction}

Deep Learning (DL) applications, such as CNNs~\cite{r50, mbnetv2, mnasnet}, transformers~\cite{vit, bert, gpt, mega-turing} and recommendation models~\cite{dlrm, dlrm_survey} have achieved superior performance in many cognitive tasks like vision, speech and language applications, which poses potentials in numerous areas like medical image analysis~\cite{medical}, photo styling~\cite{guagan}, machine translation~\cite{trans}, product recommendation~\cite{dlrm}, customized advertising~\cite{ads}, game playing~\cite{game}, \etc 
Such widespread DL applications bring great market values and lead to significant DL serving traffics. 
For example, FB has 1.82 billions of daily active users~\cite{fb_busi}. The number of advertising recommendation queries can reach 10M queries per second. 
The huge growth in consumer-generated data and use of DL services have also propelled the demand for AI-centric data centers (such as Amazon AWS~\cite{aws} and Microsoft Azure~\cite{azure}) and the increased adoption of powerful DL accelerators like GPUs.
According to the report~\cite{gpu_report}, GPU has accounted for the major share of 85\% with 2983M USD in the global data center accelerator market in 2018. And this product segment is poised to reach 29819M USD by 2025~\cite{gpu_report}.


With the ever increasing market demands, DL applications and the underlying serving hardware have demonstrate strong {scaling trends} in terms of \textbf{Computing Scaling} (\eg, increased computing parallelism, memory and storage to serve larger models) and \textbf{Model Scaling} (\eg, higher structure complexity, computing workload, parameter size for better accuracy), which greatly complicates the serving system management and optimization.
% 
% Along with the model scaling, DL hardwares also demonstrate continuous increase in their capacities. 
%
%
On the one hand, as shown in Figure~\ref{fig:scaling} (a), with the \textbf{Computing Scaling} trend, GPU with massive computing parallelism has become one of the major types of DL computing accelerators in recent data centers and maintains continuously exponential performance scaling.
Recent GPUs such as NVIDIA Tesla V100 offer 130 Tera floating point operations per second (TFLOPS), and 900 GB/s memory bandwidth, and these numbers further increase to 312 TFLOPS and 1.6TB/s memory bandwidth, which can serve tens of DL models such as ResNet50~\cite{r50} simultaneously and provide higher efficiency (Perf/Watt). 
%
On the other hand, as shown in Figure~\ref{fig:scaling} (b), \textbf{Model Scaling} has been show to be one of the most important factor in achieving better accuracy, the effectiveness of which is consistently shown in practice by industrial ultra-large models in all domains, such as vision model BiT~\cite{bit}, NLP model BERT~\cite{bert}, GPT3~\cite{gpt} and deep learning recommendation model DLRM~\cite{dlrm}.
For example, recent ultra-large model MT-NLG~\cite{mega-turing} has achieved 530 billions of parameters. Industrial-level commercial DLRMs~\cite{dlrm} have reached $\sim$TB model size, which significantly surpass single-machine memory capability and require multiple devices for collaborative computing. 


% \begin{figure*}[!t]
% 	\centering
% % 	\vspace{-2mm}
% 	\includegraphics[width=6.7in]{_figs/scaling.pdf}
% % 	\vspace{-2mm}
% 	\caption{Deep Learning {Model Scaling} and {Computing Scaling}. Such exponential scaling trends on both sides leads to {Large-scale DL Systems}.}
% 	\vspace{-2mm}
% 	\label{fig:scaling}
% \end{figure*}

{{Within such contexts, we observe the current DL system community still lacks enough awareness and attention to such \textbf{Large-scale Deep Learning Systems (LDS)},  overlooking the emerged challenges and opportunities:}}
% and leading to conservative problem settings and optimization 
    Traditional DL system optimization usually focuses on the single-model single-machine inference setting (\ie, one-to-one mapping).  However, LDS with bigger DL models and more powerful hardwares enable more flexible inference computing, bringing the many-instance to one-device, one-instance to many-device, and even many-instance to many-device mapping into practice.
%
For example, computing scaling (such as GPUs, TPUs) motivates many research works into multi-model inference on one single device, \eg, splitting one GPU into multiple containerized vGPUs or Multi-Instance GPUs (MIG) for better hardware utilization, higher serving throughput and cost efficiency. 
    Considering practical cost management (\eg, total cost of ownership, TCO), data centers serving massive inference queries also tend to migrate to {multi-tenant} inference serving, \eg, co-locating multiple inference queries on the same device, which incurs new optimization objectives (\eg, total served queries per second, QPS) and constraints (\eg, service-level agreement, SLA) from traditional single-tenant inference.
%
Similarly, the model scaling also poses requests for new one-to-many inference scenarios. The recent ultra-large model (\eg, DLRMs) incurs huge memory cost ($\sim$TB without quantization) during inference, which requires new collaborative computing paradigms such as heterogeneous computing or distributed inference. Such collaboratively serving involves remote process calls (RPCs) and low-bandwidth communications, which brings dramatically different bottlenecks from traditional single-device inference. 
    With all above scenarios involved, modern data centers face more sophisticated many-to-many scenarios and require dedicated inference query scheduling, such as service router and compute device management, for better serving performance like latency, throughput and cost, \etc


\begin{comment}
In this work, we propose a a novel computing paradigm taxonomy for ongoing LDS works, summarize the new optimization objectives, elaborate new technical design perspectives, and provide the insights for future LDS optimization.

\begin{itemize}
	\item \textbf{Multi-to-Multi Computing Paradigm} Characterized by the relations between DNN Instances (I) and Compute Devices (D), emerging LDS computing paradigms can be taxonomized into three new categories beyond Single Instance Single Device (\eph{SISD}), that is, Multi Instance Single Device (\eph{MISD}), Single Instance Multi Device (\eph{SIMD}) and Multi Instance Multi Devices (\eph{MIMD}), as shown in Figure~\ref{fig:taxonomy}.

	\vspace{1mm}
	\item \textbf{Inference Serving Oriented Objectives} Different from SISD that focuses on single-model performance, LDS works have different optimization goals, including inference \eph{latency, serving throughput, costs, scalability, quality of service}, \etc For example, multi-tenant inference (MISD) targets at improving the serving throughput and power efficiency, while super-scale model inference serving aims to enhance hardware scalability with low costs.

	
	\vspace{1mm}
	\item \textbf{At-Scale Design and Technologies} Due to the scale of inference serving, LDS works have also demonstrated many optimization challenges and opportunities within \eph{algorithm innovation}, \eph{runtime scheduling} and \eph{resource management}. For example, multi-tenant inference optimization seeks for fine-grained hardware resource partitioning and job scheduling, \eg, spatial/temporal sharing to provide QoS assurance.
	Distributed inference with slow communication bottlenecks requires dedicated model-hardware co-optimization, \eg, efficient model sharding and balanced collaboration, \etc

\end{itemize}


 
By summarizing the existing works, we aim to provide a comprehensive survey on emerging challenges, opportunities, and innovations, and thus motivates new innovations in LDS operation and optimization. 
	The rest of the survey is organized as follows:
	Section~\S\ref{sec:bg} presents the research preliminaries including our taxonomy for LDS and indicate the scope of this survey.
    Section~\S\ref{sec:misd} summarizes the challenges and recent works in multi-instance single-device (MISD) optimization;
    Section~\S\ref{sec:simd} summarizes the research works in single-instance multi-device (SIMD) optimization;
    Section~\S\ref{sec:con} concludes this work.
\end{comment}


\textbf{Definition of Multi-Tenant Computing}: 





% \newpage


% Different from traditional single model on single compute, large-scale production applications incurs degrees of more complexity regarding the \textbf{model and compute scaling}.

% \noindent $\bullet$ On the one hand, current productive applications generally require \textbf{multiple models} to accomplish one complex task. For example, Tesla Autopilot~\cite{} relies on a series of vision models like segmentation, 2D/3D detection and depth estimation to achieve the visual guidance. A full-set of perception system can have 48 DL models co-running on the single autopilot hardware set~\cite{}.
% Such \textbf{multi-model serving paradigm (or multi-tenant serving)} has drawn great attention from current compute vendors, especially on GPU hardware with great compute parallelism and resource sharing potentials. NVIDIA has recently built a series of techniques including Multi-Stream (MST)~\cite{}, Multi-Process Service (MPS)~\cite{} and Multi-Instance GPU (MIG)~\cite{} to support multi-tenant shared execution and dedicated resource partitioning for quality of service (QoS) assurance. 


% \noindent $\bullet$ On the other hand, recent DL model capacity growing speed has outpaced compute scaling (such as Moore's Law) way much and can require \textbf{multiple hosts}. For ultra-large models such as Facebook DL recommendation models (DLRM)~\cite{}, the model's resource requirements such as memory easily outnumber the single-host capacity, requiring \textbf{multiple devices} co-serving one single model. Note that such resource 
% outstripping does not only appear in training jobs, i.e., distributed training (DT)~\cite{}, but also shows up in inference job, bringing up brand new challenges and opportunities of \textbf{distributed inference (DI)}~\cite{}. 

% \noindent $\bullet$ Besides the above single compute and/or single model perspective, serving productive DL models generally relies on cloud environments (such as Amazon AWS~\cite{}, Microsoft Azure~\cite{}, Google Cloud~\cite{}) with large-scale underlying compute infrastructures, forming a even more complex large-scale \textbf{multi-model multi-device} serving problem. Such data center-based serving and management have more practical constraints (service-level latency agreement, hardware capacity requirements) and physical considerations (power efficiency, cost of serving) and raises new optimization challenges and opportunities. 


% Although multi-tasking techniques are already studied on CPUs (\eg, time slicing),  the application of bigger DL workloads and hardwares with more compute incurs new large-scale challenges.




==> _txt/3_part2.tex <==
% \newpage

\section{Model Scaling: Trending to \\ Single Instance Multi Device (SIMD)}
\label{sec:simd}


\vspace{1mm}
\subsection{Overview}

Different from MISD, the trend of SIMD is mainly brought by the tremendous model scaling~\cite{gpt,mega-turing} which makes one model hard to execute on one single machine.
For example, industrial recommendation models~\cite{dlrm} requires $\sim$TB of memory for inference.
In such cases, scaling up single machine to support such memory capacity can incur huge infrastructural cost in large-scale data centers. Therefore, one more cost-efficient way is to scale out, which is to using multiple distributed compute devices to conduct collaboratively inference.
However, unlike distributed training with long time duration and thus loose time constraints, inference serving have strict latency constraints. Thus, the communication cost in such collaboratively serving can make the SLAs more challenging to achieve. 

\vspace{1mm}
\noindent \textbf{{Enhancing Capacity Scaling}} 
The first priority of SIMD is to achieve capacity scaling of infrastructures so as to enable super-scale model inference serving. 
To do so, there are two major ways: \textbf{Scale up vs. Scale out}. 
Scale up (or vertical scaling) means upgrading or adding more resources to an system to reach a desired state of performance, \eg, more compute, memory, storage and network bandwidth, \etc
By contrast, scale out (or horizontal scaling) uses more distributed low-end machines to collaboratively serve one large DL model. SIMD such as distributed inference~\cite{fb,deepthing,hotedge,coedge} mainly uses the second scale-out solution to maintain the capacity scaling for larger DL model serving. Recently, heterogeneous inference~\cite{hm1,hm2,hm3} comes up, which combines heterogeneous resources such as hybriding CPU/GPU, hybriding cache/memory/SSD, etc. Such solutions could be considered as a scale-up solution. 

\vspace{1mm}
\noindent \textbf{{Reducing Costs}} 
For both scaling up and scaling out solutions, the major optimization targets of above solutions (\ie, SIMD) is to reduce the total cost of ownership (TCO).
For example, scaling up by increasing single machine capacity such as upgrading CPU generations, increasing memory capacity and frequencies can be expensive within large-scale data center-level infrastructures. 
Therefore, the heterogeneous inference mainly relies on existing hardwares and combines them to enhance the compute capacity, thus reducing the capacity scaling costs.
%
By contrast, scaling out utilizes multiple current generation of compute devices to serve next-generation larger models, thus also reducing the cost of setting up new dedicated hardware.
For both methods, the shared downside is that it brings complex distributed computing and communication management, and even potential performance degradation.

\begin{figure}[!b]
	\centering
% 	\vspace{-2mm}
	\includegraphics[width=3.4in]{_figs/paral.pdf}
% 	\vspace{-2mm}
	\caption{In three parallelisms, model parallelism is the common way to achieve distributed inference while the other two are only suitable for distributed training. For example, data parallelism is not suitable for inference with small batch sizes. Pipeline parallelism cannot leverage multi-node computing parallelism within a single inference request.}
% 	\vspace{-2mm}
	\label{fig:paral}
\end{figure}


\subsection{Challenges in SIMD}

\vspace{1mm}
\subsubsection{{Computing Parallelism}} 

Although SIMD with distributed devices can achieve the model's required overall capacity, distributing one entire model to collaboratively compute on multi-nodes is still very complex. 
There are many model partitioning algorithms that have been explored in {distributed training} algorithms such as data, model, and pipeline parallelism~\cite{pipelayer, pipedream, hidden}, \etc  
However, not all of them are suitable for {inference} scenarios.
As shown in Figure~\ref{fig:paral}, traditional data parallelism by splitting the batch sizes is usually not applicable since the inference serving usually comes with small batch sizes. 
Pipeline parallelism~\cite{pipelayer,pipedream,gpipe} by allocating different layers into different machines is also not suitable as it cannot achieve multi-node computing parallelism within one single inference request. 
As a result, model parallelism~\cite{hidden} is the most common way to achieve SIMD or distributed inference, as we will introduce later.


\subsubsection{{Communication Bottlenecks}} 
For model parallelism on multi-distributed machines, achieving linear or even sub-linear speedup is usually very hard. The reason is that, the major factor that influences the computing efficiency (such as latency) in model parallelism is the communication bottlenecks caused by the intermediate data transfer between different model shards (distributed nodes)~\cite{gpipe,commu1}. Depending on the data transmission speed, too much data transfer will incur significant latency overhead, \eg, with Ethernet connections in distributed machines. To avoid that, an efficient model sharding algorithm is needed to ensure the inference serving performance in MISD.
However, the intermediate data communication mechanisms vary a lot in different model architectures, such as CNNs, Transformers, and recommendation DLRMs, \etc, and thus it requires many analysis efforts and design innovations to find the optimal model sharding algorithm. 



\begin{figure*}[!t]
	\centering
% 	\vspace{-2mm}
	\includegraphics[width=6in]{_figs/fb.pdf}
	\vspace{-2mm}
	\caption{Distributed Inference could use RPCs to leverage multiple distributed hosts to collaboratively execute one large recommendation model~\cite{fb}.}
	\vspace{-2mm}
	\label{fig:fb}
\end{figure*}


\subsection{Optimization Techniques}

We mainly introduce two aspects of works that conduct SIMD: Scaling out by distributed inference and Scaling up by heterogeneous inference. 

\vspace{1mm}
\subsubsection{{Scaling Out: Distributed Inference}} 



\vspace{1mm}
\noindent \textbf{Recommendation Model Distributed Inference}
For example, recent industry-level deep learning recommendation model (DLRM)~\cite{dlrm} has reached $\sim$TB-level model size and such recommendation request takes over 79\% of Facebook's data center's workload, \cite{fb} proposed the first work that applies the distributed inference technique into the large DLRM inference serving. Different from conventional MLPs and CNNs, DLRMs are mainly composed of \eph{feature embedding tables} and fully-connected layers, where feature embedding tables are the major part of model weights (up to 80\% to 95\%). Such feature embedding part of DLRMs is memory-intensive, but have very light computation workload as it only needs to access certain columns of the embedding tables and conducts summation~\cite{fb}. 
% One example of recommendation model is shown in Figure~\ref{fig:fb} (a), and more in-depth DLRM description could be found in~\cite{dlrm_survey}.
%
% As increasing feature embedding dimensions are one of the most critical factors of enhancing model performance, single-compute memory capacity (\eg, normally up to 384GB memory for commercial devices) has greatly restricted commercial DLRM to achieve higher embedding dimensionality and better accuracy scaling. 

Therefore, distributed inference is proposed to partition large embedding tables into different compute nodes and thus overcome the inference serving memory limitation. When the table embeddings in remote nodes are required, central model could invoke remote process calls (RPCs) to directly get the computed results from remote nodes and thus fulfill the distributed inference serving.

% During this process, one problem is that although the compute results have relatively small size, the remote RPCs can still take non-negligible time compared to FC layer execution time (\eg, $\sim$ms). Therefore, one potential optimization is to derive an effective embedding table sharding based on the distributions of access patterns to reduce the RPC costs, such as identifying and allocating frequently-accessed tables (hot tables) to local machine and non-frequently accessed ones onto remote machines. 

\vspace{1mm}
\noindent \textbf{CNN Distributed Inference}
Compared to DLRMs, CNN model parallelism is more widely studied (such as channel parallelism/spatial parallelism)~\cite{hotedge} and many works have also propose the CNN models' distributed inference~\cite{coedge,deepthing}. For example, CoEdge~\cite{coedge} is one example of cooperative CNN inference with adaptive workload partitioning over heterogeneous distributed devices. Similarly, DeepThings~\cite{deepthing} also proposes a framework for adaptively distributed execution of CNN-based inference on resource constrained IoT edge devices. It designs a scalable Fused Tile Partitioning (FTP) to minimize memory footprint while exposing parallelism to collaboratively compute of major convolutional layers. It further realizes a distributed work stealing approach to enable dynamic workload distribution and balancing at inference runtime. 





\subsubsection{{Scaling Up: Heterogeneous Inference}} 


\vspace{1mm}
\noindent \textbf{Heterogeneous Memory} Besides using distributed machines, another way to address super-scale model's large memory capacity requirement is to leverage heterogeneous memory, \eg, by combining different levels of memory such as cache, main memory and even SSDs. The major challenge of such heterogeneous memory is to address the slow access speed of SSD (the access bandwidth can be usually 100x slower than memory). Targeting at this bottleneck, \cite{hm1,hm2,hm3} have proposed similar heterogeneous memory design that leverages storage-level SSDs to store partial of the embedding table weights of the DLRM. As the embedding table access patterns of DLRMs are usually sparse and have certain spatial/temporal locality, a proper embedding table placement strategy between memory/SSD with dedicated caching strategy could thus greatly enhance the heterogeneous memory access efficiency, thus reaching on-pair performance with pure memory based performance.


\vspace{1mm}
\noindent \textbf{Heterogeneous Computing} Along with heterogeneous memory, heterogeneous computing is a similar concept by hybriding the computing capacity for different processors, which is mostly commonly used for large model inference in SoCs with multiple types of computing processors such as CPU, GPU and other accelerators. For example, Synergy~\cite{synergy} proposed a HW/SW framework for high throughput CNNs on embedded heterogeneous SoC. It leverages all the available on-chip resources, which includes the dual-core ARM processor along with the FPGA and the accelerator to collaboratively compute for the CNN inference. Similar to distributed inference which partition one model onto multiple machines, heterogeneous computing also requires dedicated model sharding algorithms and co-designs the model sharding with the heterogeneous computing devices, and also considers the inter-processor communication, \etc 


% \subsection{Promising Directions} 



% \section{Multi Instance Multi Device (MIMD)}

% \noindent \textbf{Datacenter-level Task-to-Host Scheduling}


% \newpage

==> _txt/5_evaluation.tex <==
\section{Evaluation}
